Statistical inference for Linear Stochastic Approximation with Markovian Noise

In this paper we derive non-asymptotic Berry-Esseen bounds for Polyak-Ruppert averaged iterates of the Linear Stochastic Approximation (LSA) algorithm driven by the Markovian noise. Our analysis yields $\mathcal{O}(n^{-1/4})$ convergence rates to the Gaussian limit in the Kolmogorov distance. We further establish the non-asymptotic validity of a multiplier block bootstrap procedure for constructing the confidence intervals, guaranteeing consistent inference under Markovian sampling. Our work provides the first non-asymptotic guarantees on the rate of convergence of bootstrap-based confidence intervals for stochastic approximation with Markov noise. Moreover, we recover the classical rate of order $\mathcal{O}(n^{-1/8})$ up to logarithmic factors for estimating the asymptotic variance of the iterates of the LSA algorithm.

==> bootstrap.tex <==
In order to perform statistical inference with the Polyak-Ruppert estimator $\bar{\theta}_{n}$, we propose an online bootstrap resampling procedure, which recursively updates the LSA estimate as well as a large number of randomly perturbed LSA estimates, upon the arrival of each data point. The suggested procedure follows the one outlined in \cite{JMLR:v19:17-370}. It has the following advantages: it does not rely on the asymptotic distribution of the error $\sqrt{n}(\bar{\theta}_{n} - \thetas)$, does not require to know the moments of $\sqrt{n}(\bar{\theta}_{n} - \thetas)$ or its asymptotic covariance matrix $\Sigma_{\infty}$, and does not involve any data splitting.
\par 
We state the suggested procedure as follows. Let $\mathcal W^{2n} = \{W_\ell\}_{1 \leq \ell \leq 2n}$ be a set of i.i.d. random variables, independent of $\mathcal Z^{2n} = \{Z_\ell\}_{1 \leq \ell \leq 2n}$, with $\PE[W_1] = 1$ and $\var[W_1]=1$. We write, respectively, $\PPb = \PP(\cdot | \mathcal Z^{2n})$ and $\PEb = \PE(\cdot | \mathcal Z^{2n})$ for the corresponding conditional probability and expectation. In parallel with procedure \eqref{eq:lsa} that generates $\{\theta_{k}\}_{1 \leq k \leq 2n}$ and $\prtheta_{n}$, we generate $M$ independent samples $(w_{n}^{\ell},\ldots,w_{2n}^{\ell})$, $1 \leq \ell \leq M$ distributed as $\mathcal W^{2n}$, and recursively update $M$ randomly perturbed LSA estimates, that is, 
\begin{equation}
\label{eq:lsa_bootstrap}
\begin{split}
\textstyle \theta_{k}^{\boot,\ell} 
&= \textstyle \theta_{k-1}^{\boot,\ell} - \alpha_{k} w_k^{\ell}\{ \funcA{Z_k} \theta_{k-1}^{\boot,\ell} - \funcb{Z_k} \} \eqsp,~~ k \geq n+1 \eqsp, ~~ \theta_{n}^{\boot,\ell} = \theta_{n} \eqsp, \\
\textstyle \prtheta_{n}^{\boot,\ell} 
&= \textstyle n^{-1} \sum_{k=n}^{2n-1} \theta_k^{\boot,\ell} \eqsp, ~~n \geq 1 \eqsp.
\end{split}
\end{equation}
We use a short notation $\bar{\theta}_{n}^\boot$ for $\bar{\theta}_{n}^{\boot,1}$. The key idea of the procedure \eqref{eq:lsa_bootstrap} is that the "Bootstrap-world" distribution (that is, the one conditional on $\mathcal Z^{2n}$) of the perturbed samples $\sqrt n (\bar{\theta}_{n}^\boot - \bar{\theta}_n)$ is close to the distribution of the quantity of interest, that is, $\sqrt n (\bar{\theta}_n - \thetas)$. Precisely, the main result of this section will show that the quantity
\begin{equation}
\label{eq:boot_validity_supremum}
\textstyle 
\sup_{B \in \Conv(\rset^{d})} |\PPb(\sqrt n (\bar{\theta}_{n}^\boot - \bar{\theta}_n) \in B ) - \PP(\sqrt n (\bar{\theta}_n - \thetas) \in B)|
\end{equation}
is small. Although an analytic expression for $\PPb(\sqrt n (\bar{\theta}_{n}^\boot - \bar{\theta}_n) \in B )$ is not available, one can approximate it from numerical simulations according to \eqref{eq:lsa_bootstrap} by generating sufficiently large number $M$ of perturbed trajectories. Standard arguments, see e.g. \cite[Section~5.1]{shao2003mathematical} suggest that the accuracy of Monte-Carlo approximation is of order $M^{-1/2}$. To analyze the suggested procedure, we shall impose an additional assumption on the trajectory length $n$:
\begin{assum}
\label{assum:step-size-bootstrap}
Assumption \Cref{assum:step-size} holds with $\gamma = 1/2$, and $c_0 \leq 1/(\bConst{A}^2 \qcond \rme)$. Moreover, setting 
\begin{equation}
\label{eq:block_size_constraint}
\textstyle 
h(n) = \biggl\lceil \biggl(\frac{4\bConst{A}\qcond^{1/2}}{(\sqrt{2}-1)a}\biggr)^{2}(1+2\log{(2n^4)})^2 \biggr\rceil\eqsp,
\end{equation}
it holds that 
\begin{equation}
\label{eq:sample_size_bound_part_2}
\textstyle
\frac{\sqrt{n}}{h(n)} \geq \frac{2}{a(\sqrt{2}-1)} \vee \frac{c_{0}}{\alpha_{\infty}}\eqsp, \text{ and } \frac{\sqrt{n}}{\log^{2}{n}} \geq \frac{c_{0}(1 \vee \bConst{A}^2)}{a} \vee c_{0} a \bConst{A}^2  \vee \frac{4}{a c_{0}}
\end{equation}
Moreover, we assume that for $\lambda_{\min}$ defined in \eqref{eq:eig_sigma_eps} it holds that 
\begin{equation}
\label{eq:lambda_min_bound_boot}
\textstyle 
\lambda_{\min} \geq 8  \supconsteps \sqrt{\frac{\|\noisecov\| \log n}{n}} + \frac{8 (\|\noisecov\| + \supconsteps^2 )\log n}{n}
\end{equation}
\end{assum}
Note that the new bound \eqref{eq:sample_size_bound_part_2} simply states that $\sqrt{n}/\log^{2}(n)$ is sufficiently large, since $h(n)$ scales as $\log^2{n}$. We discuss the assumption \Cref{assum:step-size-bootstrap} in more details in the proof scheme. Now we formulate the main result of this section. We analyze only the setting of polynomially decaying step size with $\gamma = 1/2$, since decay rate of \eqref{eq:boot_validity_supremum} essentially depends on the approximation rate of \Cref{th:shao2022_berry}, with the fastest rate achieved when $\gamma = 1/2$. For other learning rates the decay rate of right-hand side in \Cref{th:bootstrap_validity} will be slower.

\begin{theorem}
\label{th:bootstrap_validity}
Assume \Cref{assum:iid}, \Cref{assum:noise-level}, \Cref{assum:step-size} with $\gamma = 1/2$, and \Cref{assum:step-size-bootstrap}. Then with $\PP$ -- probability at least $1 - 6/n$ it holds that
\begin{align}
&\sup_{B \in \Conv(\rset^{d})} |\PPb(\sqrt n (\bar{\theta}_{n}^\boot - \bar{\theta}_n) \in B ) - \PP(\sqrt n (\bar{\theta}_n - \thetas) \in B)| \lesssim \frac{(\bConst{A}^3 \vee 1) (1 + \supconsteps^2) \log{n}}{a^{3/2} \lambda_{\min} n^{1/4}} \\
&\qquad + \frac{\sqrt{d}}{\sqrt{n}}\left(\frac{\supconsteps^3}{\lambda_{\min}^{3/2}} + \supconsteps \frac{\sqrt{\log{n}}}{\sqrt{\lambda_{\min}}} + \frac{(1 + \supconsteps^2 / \lambda_{\min}) \log{n}}{\sqrt{n}} \right) + \frac{\Remainder_{2}\rme^{-(c_0/2) a \sqrt{n}}}{\lambda_{\min}}\norm{\theta_0-\thetas}\eqsp,
\end{align}
where $\Remainder_{2} = \Remainder_{2}(n,a,\bConst{A},\supconsteps)$ is a polynomial function defined in \eqref{eq:remainders_theorem_bootstrap}.
\end{theorem}

The proof of \Cref{th:bootstrap_validity} is based on the Gaussian approximation performed both in the "real" world and bootstrap world together with an appropriate Gaussian comparison inequality. The main steps of the proof are illustrated by the following scheme:

\begin{tikzcd}[column sep = 120pt]
\text{Real world: \quad\quad} \sqrt n \bA(\bar{\theta}_{n} - \thetas) \arrow[<->]{r}{\text{Gaussian approximation, Th.}~\ref{th:shao2022_berry}}  &
  \xi \sim \mathcal N(0,  \noisecov )  \arrow[<->]{d}{\text{Gaussian comparison, Theorem }\ref{prop: gaussian comparison}} 
\\
\text{Bootstrap world: } \sqrt n \bA (\bar{\theta}_{n}^\boot - \bar{\theta}_n) \arrow[<->]{r}{\text{Gaussian approx. in Bootstrap world, Th.}~\ref{CLT in the bootstrap world}} &
\xi^\boot \sim \mathcal N(0,  \noisecov^\boot) 
\end{tikzcd}

In the above scheme we have denoted by $ \noisecov^\boot = n^{-1} \sum_{\ell = n}^{2n-1} \funnoisew_\ell \funnoisew_\ell^{\top}$ the sample covariance matrix approximating $\noisecov$. 
Gaussian approximation for the true distribution of $\sqrt n \bA(\bar{\theta}_{n} - \thetas)$ follows from \Cref{th:shao2022_berry}. Proof of Gaussian approximation in the Bootstrap world \Cref{CLT in the bootstrap world} is also based on the inequality \eqref{eq:shao_zhang_bound}, but is more complicated and involves the expansion analysis of the LSA error from \cite{aguech2000perturbation}. This technique allows to separate the LSA error into different scales with respect to the step sizes $\{\alpha_{k}\}$, see \Cref{sec:error_decomspotion_perturbed} for details. However, this technique requires to impose additional assumption \Cref{assum:step-size-bootstrap} - eq. \eqref{eq:sample_size_bound_part_2}. Proof of the Gaussian comparison part of \Cref{prop: gaussian comparison} is based on Pinsker's inequality and matrix Bernstein inequality. The latter result requires that $n$ is large enough to ensure that minimal eigenvalue of $\noisecov^\boot$ is close to $\lambda_{\min}$, justifying the assumption \Cref{assum:step-size-bootstrap} - eq. \eqref{eq:lambda_min_bound_boot}. Detailed proof if provided in \Cref{appendix:bootstrap}.

\textbf{Discussion.} We emphasize that the Gaussian approximation result of \Cref{th:shao2022_berry} (with Bootstrap world generalization in \Cref{CLT in the bootstrap world}) is a key result to prove the above bootstrap validity. This argument was missing in the earlier works studying confidence intervals for stochastic optimization algorithms \cite{chen2020aos,zhu2023online_cov_matr,zhong2023online}, where the authors considered procedures to estimate $\Sigma_{\infty}$ in \eqref{eq:asympt_cov_matr}. They combine \emph{non-asymptotic} bounds on the accuracy of recovering $\Sigma_{\infty}$ with only \emph{asymptotic} validity of the resulting confidence intervals. We expect that our proof technique for \Cref{th:shao2022_berry} can be used to provide similar non-asymptotic validity results for outlined approaches for constructing confidence intervals based on the estimation of the asymptotic covariance matrix.

\begin{corollary}(Set of Euclidean balls or ellipsoids) Suppose that we are interested in estimating quantile of a given order $\alpha \in (0,1)$ and some matrix $B \in \rset^{d \times d}$, that is, the quantity
\begin{equation}
\label{eq: real quantile}
t_\alpha = \inf\{ t > 0: \PP(\sqrt n \|B(\bar{\theta}_{n} - \thetas)\| \geq t) \leq \alpha \}.
\end{equation}
We define its counterpart in the Bootstrap world, $t_\alpha^\boot$, as
\begin{equation}
\label{eq: boot quantile}
t_\alpha^\boot = \inf\{ t > 0: \PPb(\sqrt n \|B(\bar{\theta}_{n}^\boot - \bar{\theta}_n)\| \geq t) \leq \alpha \}. 
\end{equation}
Note that $t_\alpha^\boot$ is defines with respect to the bootstrap measure, therefore, it depends on the date $\mathcal Z^{2n}$. This bootstrap critical value $t_\alpha^\boot$ is applied in the Bootstrap world to build the confidence set 
\begin{equation}
\label{confidence set}
\mathcal E(\alpha) = \{\theta \in \rset^d: \sqrt n \| B(\theta - \bar{\theta}_n)\| \leq t_\alpha^\boot\}\eqsp.
\end{equation}
\Cref{th:bootstrap_validity} justifies this construction and evaluate the coverage probability of the true value $\thetas$ by this set. It states that 
$$
\PP(\thetas \notin \mathcal E(\alpha)) = \PP(\sqrt n \|B(\bar{\theta}_n - \thetas)\| > t_\alpha^\boot) \approx \alpha\eqsp,
$$
with the error of order $n^{-1/4}$ in the right-hand side. Although an analytic expression for $t_\alpha^\boot$ is not available, one can approximate it by generating a large number $M$ of independent samples of $\mathcal W_n$ and computing from them the empirical distribution function of $\sqrt n \|B(\bar{\theta}_{n}^\boot - \bar{\theta}_n)\|$, following \eqref{eq:lsa_bootstrap}.
\end{corollary}

\begin{remark}
\label{rem:non-linear}
A natural question that arises after \Cref{th:bootstrap_validity} is whether it is possible to prove the same bounds for non-linear problems, e.g. for the iterates of stochastic optimization algorithms. Since there is a number of MSE bounds for corresponding algorithms with explicit dependence on the step size $\alpha_{k}$, see e.g. \cite{moulines2011non,bach:moulines:2013}. Therefore, we expect that it is possible to obtain a counterpart to \Cref{th:shao2022_berry}. At the same time, for stochastic optimization, unlike LSA, there is no direct counterpart to the perturbation expansion analysis of \cite{aguech2000perturbation}, which makes it more difficult to prove the counterpart of \Cref{th:bootstrap_validity}. Similarly, we would like to emphasize that the generalizations of the procedure \eqref{eq:lsa_bootstrap} for the case where $\{\State_k\}_{k \in \nset}$ are not independent, e.g. form a Markov chain, are also complicated since \eqref{eq:shao_zhang_bound} is only valid for independent observations $\xi_{\ell}$.
\end{remark}







==> experiments.tex <==
We illustrate our findings for the setting of temporal difference (TD) learning algorithm \cite{sutton1988learning,sutton:book:2018} for policy evaluation in RL. Compared to the previously considered applications in \cite{samsonov2024gaussian}, in our example we use the TD learning algorithm with Markovian noise observations in \emph{offline} setting, that is, when the data policy is different. In the TD algorithm we consider a discounted MDP (Markov Decision Process) given by a tuple $(\S,\A,\PMDP,r,\gamma)$. Here $\S$ and $\A$ stand for state and action spaces and $\gamma \in (0, 1)$ is a discount factor. Assume $\S$ is a complete metric space with metric $\metrics$ and Borel $\sigma$-algebra $\borel{\S}$. $\PMDP$ stands for the transition kernel $\PMDP(B | s,a)$, which determines the probability of moving from state $s$ to a set $B \in \borel{\S}$ when action $a$ is performed. Reward function $r\colon \S \times \A \to [0,1]$ is assumed to be deterministic. \emph{Policy} $\pi(\cdot|s)$ is the distribution over action space $\A$ corresponding to agent's action preferences in state $s \in \S$. We aim to estimate \emph{value function}
\[
\textstyle
V^{\pi}(s) = \PE[\sum_{k=0}^{\infty}\gamma^{k}r(s_k,a_k)|s_0 = s]\eqsp,
\]
where $a_{k} \sim \pi(\cdot | s_k)$, and $s_{k+1} \sim \PMDP(\cdot | s_{k}, a_{k})$ for any $k \in \nset$. Define the transition kernel under $\pi$,
\begin{equation}
\label{eq:transition_matrix_P_pi}
\textstyle \PMDP_{\pi}(B | s) = \int_{\A} \PMDP(B | s, a)\pi(\rmd a|s)\eqsp,
\end{equation}
which corresponds to the $1$-step transition probability from state $s$ to a set $B \in \borel{\S}$. The state space $\S$ here can be arbitrary. It is a common option to consider the \emph{linear function approximation} for $V^{\pi}(s)$, defined for $s \in \S$, $\theta \in \rset^{d}$, and a feature mapping $\varphi\colon \S \to \rset^{d}$ as $V_{\theta}^{\pi}(s) =  \varphi^\top(s) \theta$. Here $d$ is the dimension of feature space. Our goal is to find a parameter $\thetas$ that defines the best linear approximation of $V^{\pi}$ \cite{tsitsiklis:td:1997} in the following sense. We denote by $\mu$ the invariant distribution over the state space $\S$ induced by $\PMDP^{\pi}(\cdot | s)$ in \eqref{eq:transition_matrix_P_pi}. Then we define $\thetas$  as a solution to the problem
\begin{equation}
\label{eq:def:theta}
\textstyle \thetas = \arg\min_{\theta \in \rset^d}\PE_{\mu}\bigl[\left( V^{\pi}_{\theta}(s) - V^{\pi}(s) \right)^2\bigr].
\end{equation}

\tcr{Here should be assumptions for td learning}
\begin{comment}
We define the \emph{design matrix} $\covfeat$ as
\begin{equation}
\label{eq:covfeat_matr_def}
\textstyle
\covfeat = \PE_{\mu}[\varphi(s)\varphi(s)^{\top}] \in \rset^{d \times d}\eqsp.
\end{equation}
\end{comment}

In the setting of linear function approximation the estimation of $V^{\pi}(s)$ reduces to the estimation of $\thetas \in \rset^{d}$, which can be done via the LSA procedure. Here we define starting state to be $s_0$ and $k$-th step randomness is given by the tuple $\State_k = (s_k, a_k, s_{k+1})$. Where $a_k \sim \pi(\cdot|s_k)$ and $s_{k+1} \sim P(\cdot|s_k,a_k)$. Then the corresponding LSA update can be written as
\begin{equation}
\label{eq:LSA_procedure_TD}
\textstyle 
\theta_{k} = \theta_{k-1} - \alpha_{k} (\funcAw_{k} \theta_{k-1} - \funcbw_{k})\eqsp,
\end{equation}
where $\funcAw_{k}$ and $\funcbw_{k}$ are given, respectively, by
\begin{equation}
\label{eq:matr_A_def}
\textstyle \funcAw_{k} =  \phi(s_k)\{\phi(s_k) - \gamma \phi(s_{k+1})\}^{\top}\eqsp, \quad \funcbw_{k} = \textstyle \phi(s_k) r(s_k,a_k)\eqsp.
\end{equation}

\subsection{Numerical results of FrozenLake RL Environment}

We consider the Frozenlake environment from OpenAI gym \cite{brockman2016openai}. In the setting the RL agent controls movement of a character on a $8 \times 8$ grid. A reward of $1$ is awarded if the character reaches the target tile and reward for any other state transition is $0$. Each other tile is either walkable or absorbing. 

We consider associated MDP and aim to evaluate the
value function of the nearly optimal policy $\pi(\cdot|s)$ trained using Q-learning.  We consider problem of approximate problem evaluation in this MDP using TD learning algorithm. We consider feature mapping $\phi(s) = v_s$, where $v_s \sim \gauss(0, I_d)$. We set $d=3$ for our numerical results. We run the procedure \eqref{eq:LSA_procedure_TD} with learning rates $\alpha_k = c_0/k^{\gamma}$ where we set $\gamma=\frac{2}{3}$ as it is suggested to be the optimal learning rate. For the experiments we aim to estimate the supremum
\begin{equation}
\label{eq:approx_supremum_experiment}
\textstyle 
\Delta_{n} := \sup_{x \in \rset} \bigl|\P(\sqrt{n} \left(\bar{\theta}_{n} - \thetas\right)^{\top}u \leq x) - \P(\eta \leq x)\bigr|\eqsp,
\end{equation}
where $\eta \sim \gauss(0, \norm{V_{\infty}^{\frac{1}{2}} u})$ and $u = \phi(s_0)$ is vector corresponding to the starting state projection. Second, for $n \in \{200, \ldots, 1638400\}$, where next sample size is twice larger than the previous one, we generate $N = 327680$ trajectories of TD algorithm and approximate the distribution of $\sqrt{n}\left(\bar{\theta}_{n} - \thetas\right)^{\top}u$ based on the corresponding empirical distribution. We also implement OBM procedure as described in \eqref{eq:sigma_hat_variance} to find exact distribution of $\hat{\theta}_{n,b_n}(u)$ and compare the convergence rate of OBM estimator distribution to theoretical distribution. To do that we compare empirical distribution of $\sqrt{n}\left(\bar{\theta}_n - \thetas\right)^{\top}u$ to distribution of $\eta$ and distribution of $\hat{\theta}_{n,b_n}(u) \sim \gauss(0, \hat{\sigma}^2(u))$ and calculate corresponding Kolmogorov distances.

\begin{figure}[t!]
\centering
\subfigure{\includegraphics[width=1.0\linewidth]{figures/kolmogorov_dist_obm.pdf}}%
\vspace{-3mm}
\caption{Kolmogorov distance of empirical distributions of td learning algorithm to asymptotic covariance distribution and OBM estimation distributions. }
\label{fig:kolmogorov-distance}
\vspace{-3mm}
\end{figure}

\begin{figure}[t!]
\centering
\subfigure{\includegraphics[width=1.0\linewidth]{figures/obm-plots.png}}%
\vspace{-3mm}
\caption{Empirical distribution from td learning algorithm compared with OBM estimation distributions. Figures a), b), c), d) show comparison with distributions with number of iterations equal to $1600$, $12800$, $102400$, $1638400$ correspondingly.}
\label{fig:kolmogorov-distance}
\vspace{-3mm}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabularx}{\textwidth}{c *{6}{>{\centering\arraybackslash}X}}
\toprule
 & \multicolumn{6}{c}{\textbf{Confidence levels}} \\ 
 & \multicolumn{2}{c}{\textbf{0.95}}  & \multicolumn{2}{c}{\textbf{0.85}}  & \textbf{0.75} \\ 
\boldmath{$n$} & median & stddev & median & stddev & median & stddev \\
\midrule
1600 & 0.998 & 0.030 & 0.984 & 0.069 & 0.950 & 0.108 \\
\midrule
12800 & 0.995 & 0.017 & 0.962 & 0.042 & 0.903 & 0.068 \\
\midrule
102400 & 0.979 & 0.042 & 0.911 & 0.066 & 0.825 & 0.080 \\
\midrule
1638400 & 0.983 & 0.014 & 0.920 & 0.022 & 0.839 & 0.027 \\
\bottomrule
\end{tabularx}
\vspace{-3mm}
\caption{Coverage probabilities of OBM estimation for the empirical distribution. }
\label{table:coverage-probabilities}
\end{table}


